Influence of N,N,N-trimethyl-1-adamantyl ammonium (TMAda+) Structure Directing Agent on Al Pair Distributions and Features in Chabazite Zeolite

While organic structure directing agents (OSDAs) are well known to have a directional influence on the topology of a crystallizing zeolite, the relationship between OSDA charge and siting of aliovalent ions on a primarily siliceous framework is unclear. Here, we explore the relationship between OSDA orientation, Al3+ siting, and lattice energy, taking as a model system CHA zeolite occluded with N,N,N-trimethyl-1-adamantyl ammonium (TMAda+) at an Si/Al ratio of 11/1. We use density functional theory calculations to parametrize a fixed-charge classical model describing van der Waals and electrostatic interactions between framework and OSDA. We enumerate and explore all possible combinations of OSDA orientation and Al location (attending to Lowenstein's rule) within a 36 T-site supercell. We find that interaction energies vary over 60 kJ/double-six-ring-unit (d6r). Further, analysis of configurations reveals that energies are sensitive to Al-Al proximity, such that low energies are associated with Al3+ pairs in 8-membered rings and higher energies associated with Al3+ pairs in smaller 6- and 4-membered rings. Comparisons with Al siting inferred from CHA zeolite crystallized with TMAda+ suggests that these computed interaction energies are useful reporters of observed Al siting in CHA synthesized with TMAda+.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
